Thermophysical modeling of main-belt asteroids from WISE thermal data

By means of a varied-shape thermophysical model (VS-TPM) of Hanus et al. (2015) that takes into account asteroid shape and pole uncertainties, we analyze the thermal IR data acquired by the NASA's WISE satellite of about 300 asteroids with derived convex shape models. We utilize publicly available convex shape models and rotation states as input for the TPM. For more than one hundred asteroids, the TPM gives us an acceptable fit to the thermal IR data allowing us to report their size, thermal inertia, surface roughness or visible geometric albedo. This work more than doubles the number of asteroids with determined thermophysical properties. In the remaining cases, the shape model and pole orientation uncertainties, specific rotation or thermophysical properties, poor thermal IR data or their coverage prevent the determination of reliable thermophysical properties. Finally, we present the main results of the statistical study of derived thermophysical parameters within the whole population of main-belt asteroids and within few asteroid families. Our sizes are, in average, consistent with the radiometric sizes reported by Mainzer et al. (2016). The thermal inertia increases with decreasing size, but a large range of thermal inertia values is observed within the similar size ranges between D~10-100 km. We derived unexpectedly low thermal inertias (<20 SI) for several asteroids with sizes 10<D<50 km, indicating a very fine and mature regolith on their surface. The thermal inertia values seem to be consistent within several collisional families. The fast rotators with P<4 h tend to have slightly larger thermal inertia values, so probably are not covered by a fine regolith. This could be explained, for example, by the loss of the fine regolith due to the centrifugal force, or by the ineffectiveness of the regolith production (e.g., by the thermal cracking mechanism of Delbo' et al. 2014).

==> tab/tab_models.tex <==
%\onecolumn
%\scriptsize{
\begin{table*}
\caption{\label{tab:models}List of asteroid models derived by the lightcurve inversion method that we use for the TPM modeling. For each asteroid, the table gives the ecliptic coordinates $\lambda$ and $\beta$ of the pole solutions, the sidereal rotational period $P$, the number of dense lightcurves $N_{\mathrm{lc}}$ observed during $N_{\mathrm{app}}$ apparitions, the number of sparse data points from USNO-Flagstaff $N_{\mathrm{689}}$ and Catalina Sky Survey $N_{\mathrm{703}}$, and the reference.}
\begin{tabular}{r@{\,\,\,}l rrrr D{.}{.}{6} ccccc}
\hline 
\multicolumn{2}{c} {Asteroid} & \multicolumn{1}{c} {$\lambda_1$} & \multicolumn{1}{c} {$\beta_1$} & \multicolumn{1}{c} {$\lambda_2$} & \multicolumn{1}{c} {$\beta_2$} & \multicolumn{1}{c} {$P$} & $N_{\mathrm{lc}}$ & $N_{\mathrm{app}}$  & $N_{\mathrm{689}}$ & $N_{\mathrm{703}}$ & Reference \\
\multicolumn{2}{l} { } & [deg] & [deg] & [deg] & [deg] & \multicolumn{1}{c} {[hours]} &  &  &  &  & \\
\hline\hline
624 & Hektor & 331 & $-$32 &  &  & 6.92051 & 17 & 8 &  &  & \citet{Kaasalainen2002c} \\
624 & Hektor & 333* & $-$32* & 135 & $-$16 & 6.920509 & 19 & 9 & 201 & 56 & Revised \\

1036 & Ganymed & 214 & $-$73 &  &  & 10.313 & 21 & 1 &  &  & \citet{Kaasalainen2002b} \\
1036 & Ganymed & 190 & $-$78 &  &  & 10.31284 & 177 & 4 & 155 & 20 & Revised \\

1627 & Ivar & 338 & 40 &  &  & 4.79517 & 56 & 4 &  &  & \citet{Kaasalainen2004b} \\
1627 & Ivar & 334 & 39 &  &  & 4.79517 & 83 & 4 & 68 & 152 & Revised \\

1865 & Cerberus & 292 & $-$72 &  &  & 6.803284 & 28 & 8 &  &  & \citet{Durech2012b} \\
1865 & Cerberus & 311 & $-$78 &  &  & 6.80329 & 47 & 8 &  & 62 & Revised \\

1980 & Tezcatlipoca & 334 & $-$65 &  &  & 7.25226 & 48 & 5 &  &  & \citet{Kaasalainen2004b} \\
1980 & Tezcatlipoca & 324 & $-$69 &  &  & 7.25226 & 49 & 6 & 29 & 35 & Revised \\
\hline
\end{tabular}
*Preferred solution by \citet{Marchis2014}.
\end{table*}
%\tablefoot{
%}
%}

==> tab/tab_phi0.tex <==
\begin{table}
\caption{\label{tab:phi0}Expected uncertainties of the rotational phase $\delta\phi_0$ and the optimized values of the rotational phase $\phi_0$ by the TPM for shape models from the DAMIT and revised shape models.}
\centerline{
\begin{tabular}{r@{\,\,\,}lcccc} \hline
\multicolumn{2}{c} {Asteroid} & \multicolumn{2}{c} {DAMIT shape}  & \multicolumn{2}{c} {Revised shape} \\
  &  & $\delta\phi_0$ [deg] & $\phi_0$ [deg] & $\delta\phi_0$ [deg] & $\phi_0$ [deg] \\ \hline\hline
624  & Hektor & 18 & $-$6 & 10 & 3 \\
1036  & Ganymed & 540 & 18 & 10 & 9 \\
1627  & Ivar & 16 & 3 & 10 & 9 \\
1865  & Cerberus & 10 & 12 & 10 & $-$9 \\
1980  & Tezcatlipoca & 20 & $-$2 & 10 & $-$3 \\
\end{tabular}
}
\end{table}

